Spectral deferred corrections with fast-wave slow-wave splitting

The paper investigates a variant of semi-implicit spectral deferred corrections (SISDC) in which the stiff, fast dynamics correspond to fast propagating waves ("fast-wave slow-wave problem"). We show that for a scalar test problem with two imaginary eigenvalues $i \lambda_{fast}$, $i \lambda_{slow}$, having $\Delta t \left(\left| \lambda_{fast} \right| + \left| \lambda_{slow} \right| \right) < 1$ is sufficient for the fast-wave slow-wave SDC (FWSW-SDC) iteration to converge and that in the limit of infinitely fast waves the convergence rate of the non-split version is retained. Stability function and discrete dispersion relation are derived and show that the method is stable for essentially arbitrary fast-wave CFL numbers as long as the slow dynamics are resolved. The method causes little numerical diffusion and its semi-discrete phase speed is accurate also for large wave number modes. Performance is studied for an acoustic-advection problem and for the linearised Boussinesq equations, describing compressible, stratified flow. FWSW-SDC is compared to a diagonally implicit Runge-Kutta (DIRK) and IMEX Runge-Kutta (IMEX) method and found to be competitive in terms of both accuracy and cost.

==> app.tex <==
\section*{Appendix}
\todo{remove this from an actual submission; maybe leave it as part of arxiv preprint}
We adopt the proof for the local truncation error of SDC based on either implicit or explicit Euler~\cite{ShuEtAl2007} to prove the following for the local truncation error for IMEX-SDC.
\begin{theorem}
If the solution $u$ is sufficiently smooth and $f$ is Lipshitz-continuous, the local truncation error for the fast-wave slow-wave SDC method with $M$ nodes and $k$ iterations is
\begin{equation}
	\text{LTE} = \left| u(\tau_m) - u^k_m \right| = \mathcal{O}(h^{\min[k+1,P+1])})
\end{equation}
for $m=1,\ldots,M$ where $P$ is the order of the used quadrature rule.
\end{theorem}
\begin{proof}
The proof works by induction over $k$ and $m$.
As preparation, we note that the continuous form of the node-to-node equation can be derived by taking the difference of~\eqref{eq:picard} for $t = \tau_{m+1}$ and $t = \tau_m$, which gives
\begin{equation}
	\label{eq:picard_node_to_node}
	u(\tau_{m+1}) = u(\tau_m) + \int_{\tau_m}^{\tau_{m+1}} f(u(s))~ds.
\end{equation}
\\
\emph{Base case:} Here, we show that the assumption is true for any $k \geq 0$ for $m=0$ and for $m=1,\ldots,M$ if $k=0$.
Because $u^k_0 = u_0$ by construction and $u_0 = u(t_0)$ by the localizing assumption, it trivially holds that
\begin{equation}
 	\left| u(\tau_0) - u^k_0 \right| = 0 = \mathcal{O}(h^{k+1}) \ \text{for} \ k\geq0.
\end{equation}
Furthermore, SDC is initialized by copying $u_0$ to all intermediate solutions, so that $u^0_m = u_0$ by construction. Then, using a Taylor expansion,
\begin{equation}
	u(\tau_m) - u^0_m = u(\tau_0) + \tau_m u'(\tau_0) + \mathcal{O}(\tau_m^2) - u^0_m
	\ \text{for}~m=1,\ldots,M.
\end{equation}
Since $u(\tau_0) = u^0_m$ and $\tau_m \leq h$ we get
\begin{equation}
	\left| u(\tau_m) - u^0_m \right| = \mathcal{O}(h^1) \ \text{for} \ m=1,\ldots,M.
\end{equation}
Because $P \geq 0$, this proves the base case.\\
\emph{Hypothesis (from $k$ to $k+1$):} The induction hypothesis is that for $0 \leq k' \leq k$ we have
\begin{equation}
	\label{eq:assump1}
	\left| u(\tau_m) - u^{k'}_{m} \right| = \mathcal{O}(h^{\min[k'+1,P+1]}) \ \text{for} \ m=1,\ldots,M
\end{equation}
and that for $k+1$ we have
\begin{equation}
	\label{eq:assump2}
	\left| u(\tau_{m'}) - u^{k+1}_{m'} \right| = \mathcal{O}(h^{\min[k+2,P+1]})
	\ \text{for} \ 0 \leq m' \leq m.
\end{equation}
\emph{Induction step:} We now show that then also
\begin{equation}
	\left| u(\tau_{m+1}) - u^{k+1}_{m+1} \right| = \mathcal{O}(h^{\min[k+2,M+1]})
\end{equation}
holds.
By subtracting~\eqref{eq:sdc} from~\eqref{eq:picard_node_to_node} and using the triangle inequality, we get
\begin{align*}
	\left| u(\tau_{m+1}) - u_{m+1}^{k+1} \right| &\leq 
	\left| u(\tau_m) - u_m^{k+1} \right| 
	+ \Delta \tau_m \left| \ffast(u^{k+1}_{m+1}) - \ffast(u^{k}_{m+1}) \right| 
 + \Delta \tau_m \left| \fslow(u^{k+1}_m) - \fslow(u^k_m) \right| \\
						         &\quad + \left| \int_{\tau_m}^{\tau_{m+1}} f(s)~ds - I_{m}^{m+1}(\mathbf{u}) \right|.
\end{align*}
By~\eqref{eq:assump2}, the first term on the right hand side is $\mathcal{O}(h^{\min[k+2,P+1]})$.
By Lipshitz continuity of $f$, we have for the explicit, slow term
\begin{align*}
	\Delta \tau_m \left| \fslow(u^{k+1}_m) - \fslow(u^{k}_{m}) \right| 
	&\leq  \Delta \tau_m L \left| u^{k+1}_{m} - u^{k}_{m} \right| \\
	&\leq  \Delta \tau_m L \left| u^{k+1}_m - u(\tau_m) \right| + \Delta \tau_m L \left| u(\tau_m) - u^{k}_{m} \right| \\
	&=  \mathcal{O}(h^{\min[k+2,P+1]}) + \mathcal{O}(h^{\min[k+1,P+1]})
\end{align*}
using~\eqref{eq:assump1} and~\eqref{eq:assump2}.
The fast implicit term can be estimated by
\begin{align*}
	\Delta \tau_m \left| \ffast(u^{k+1}_{m+1}) - \ffast(u^k_{m+1}) \right| 
	&\leq \Delta \tau_m L \left| u^{k+1}_{m+1} - u^k_{m+1} \right| \\
	&\leq \Delta \tau_m L \left| u^{k+1}_{m+1} - u(\tau_{m+1}) \right| + \Delta \tau_m L \left| u(\tau_{m+1}) - u^{k}_{m+1} \right| \\
	&= \Delta \tau_m L \left| u^{k+1}_{m+1} - u(\tau_{m+1}) \right|  + \mathcal{O}(h^{\min[k+1,P+1]})
\end{align*}
using~\eqref{eq:assump1}.
Putting all together gives
\begin{equation}
	\left| u^{k+1}_{m+1} - u(\tau_{m+1}) \right| \leq \mathcal{O}(h^{\min[k+1,P+1]}) + \Delta \tau_m L \left| u^{k+1}_{m+1} - u(\tau_{m+1}) \right|  +  \mathcal{O}(h^{P+1})
\end{equation}
Without loss of generality we can assume that the time step $h$ is small enough such that $\Delta \tau_m L_{\text f} < 1$. 
Then, it follows that
\begin{equation}
	\left(1 - \Delta \tau_m L \right) \left| u^{k+1}_{m+1} - u(\tau_{m+1}) \right| \leq \mathcal{O}(h^{\min[K+1,P+1]})
\end{equation}
and thus
\begin{equation}
	 \left| u^{k+1}_{m+1} - u(\tau_{m+1}) \right| = \mathcal{O}(h^{\min[K+1,P+1]})
\end{equation}
\end{proof}
